Distribution-dependent and Time-uniform Bounds for Piecewise i.i.d Bandits

We consider the setup of stochastic multi-armed bandits in the case when reward distributions are piecewise i.i.d. and bounded with unknown changepoints. We focus on the case when changes happen simultaneously on all arms, and in stark contrast with the existing literature, we target gap-dependent (as opposed to only gap-independent) regret bounds involving the magnitude of changes $(\Delta^{chg}_{i,g})$ and optimality-gaps ($\Delta^{opt}_{i,g}$). Diverging from previous works, we assume the more realistic scenario that there can be undetectable changepoint gaps and under a different set of assumptions, we show that as long as the compounded delayed detection for each changepoint is bounded there is no need for forced exploration to actively detect changepoints. We introduce two adaptations of UCB-strategies that employ scan-statistics in order to actively detect the changepoints, without knowing in advance the changepoints and also the mean before and after any change. Our first method \UCBLCPD does not know the number of changepoints $G$ or time horizon $T$ and achieves the first time-uniform concentration bound for this setting using the Laplace method of integration. The second strategy \ImpCPD makes use of the knowledge of $T$ to achieve the order optimal regret bound of $\min\big\lbrace O(\sum\limits_{i=1}^{K} \sum\limits_{g=1}^{G}\frac{\log(T/H_{1,g})}{\Delta^{opt}_{i,g}}), O(\sqrt{GT})\big\rbrace$, (where $H_{1,g}$ is the problem complexity) thereby closing an important gap with respect to the lower bound in a specific challenging setting. Our theoretical findings are supported by numerical experiments on synthetic and real-life datasets.

==> contribution.tex <==
Our contributions are mainly three fold. First, we propose two actively adaptive upper confidence bound (UCB) algorithms, referred to as UCB-Changepoint Detection (UCB-CPD) and Improved Changepoint Detector (ImpCPD), which try to locate the changepoints in the distribution and adapt accordingly to minimize the cumulative regret. Our algorithms try to minimize the regret by quickly detecting small enough changepoint gaps and within two changepoints they quickly find the optimal arm. UCB-CPD is an anytime algorithm whereas ImpCPD is the first phase-based algorithm for this setting. Secondly, we analyze these algorithms theoretically and prove the gap-dependent regret upper bound that consist of both the changepoint gaps ($\Delta^{chg}_{i,g}$) as well as the optimality gaps ($\Delta^{opt}_{i,g}$) for each changepoint $g=1,2,\ldots,G$, $i\in\A$. In stark contrast, DUCB, SWUCB, and CUSUM only consider the minimum optimality gap ($\Delta^{opt}_{\min}$) over the entire horizon to prove their regret bounds, which scales very badly with a large number of changepoints $G$ and large horizon $T$. This is shown in Table \ref{tab:comp-bds} in the special case when all the gaps are same such that for all $i\in\A,g\in\G$, $\Delta^{opt}_{i,g} = \Delta^{chg}_{i,g} =  \Delta^{opt}_{\min}$ and $H^{opt}_g = \frac{K}{(\Delta^{opt}_{\min})^2}$. We also prove the gap-dependent and independent lower bound for an optimal oracle policy $\pi^*$ as opposed to \citet{garivier2011upper} which proves a lower bound for a policy $\pi$ only when $G=2$. Thirdly, we prove gap-independent regret upper bound of $O( \sqrt{GT}\log T)$ for UCB-CPD and an order optimal regret upper bound of $O( \sqrt{GT})$ for ImpCPD algorithm with the additional knowledge of $T$. Hence, ImpCPD has the best theoretical guarantees than all the existing algorithms (see Table \ref{tab:comp-bds}). We show that UCB-CPD and ImpCPD perform very well across diverse piecewise i.i.d environments. In all the environments considered ImpCPD outperforms all the passively adaptive and actively adaptive algorithms except the oracle algorithms. Also, both our algorithms do not require the knowledge of the number of changepoints $G$ for optimal performance and UCB-CPD also does not require the knowledge of horizon $T$ as opposed to other algorithms (see Table \ref{tab:comp-bds}: column 5,6). A detailed table on gap-dependent bound can be found in Table \ref{tab:comp-GD-bds}, Appendix \ref{regret-table}.




\begin{table}[!th]
\begin{center}
%\begin{tabular}{p{18em}p{18em}}
\vspace*{-1.5em}
%\begin{tabular}{p{30em}}
\caption{Regret Bound of Algorithms}
\label{tab:comp-bds}
%\begin{tabular}{p{5em}p{3em}p{7em}}
\begin{tabular}{|p{4 em}|p{1em}|p{10em}|p{7em}|p{1em}|p{1em}|}
\toprule
Algorithm  &   \hspace*{1mm}Type &Gap-Dependent & Gap-Independent & T & G \\
\hline
ImpCPD        & A &$O\big(\sum\limits_{g=1}^G\dfrac{\log({T}/{H^{opt}_{g}})}{(\Delta^{opt}_{\min})}\big)$ & $O\left(\sqrt{GT}\right)$ & Y & N\\
UCB-CPD        & A &$O\big(\sum\limits_{g=1}^G\dfrac{\log T}{(\Delta^{opt}_{\min})}\big)$ & $O\left(\sqrt{GT}\log T\right)$ & N & N \\%\midrule
CUSUM             & A &$O\big(\dfrac{G\log T}{(\Delta^{opt}_{\min})}\big)$& $O\left( \sqrt{GT\log \frac{T}{G}}\right)$ & Y & Y \\%\midrule
EXP3.R         & A &N/A& $O\left( G\sqrt{T\log T}\right)$ & Y & N\\%\midrule
DUCB        & P &$O\big(\dfrac{\sqrt{GT}\log T}{(\Delta^{opt}_{\min})}\big)$& $O\left(\sqrt{GT}\log T\right)$ & Y & Y\\
SWUCB         & P &$O\big(\dfrac{\sqrt{GT\log T}}{(\Delta^{opt}_{\min})}\big)$& $O\left(\sqrt{GT\log T}\right)$ & Y & Y\\%\midrule
Lower Bound         & O &$O\big(\sum\limits_{g=1}^G\dfrac{ \log ({T}/{(GH^{opt}_g)})}{\Delta^{opt}_{\min}}\big)$ & $\Omega\left( \sqrt{GT}\right)$ & Y & Y\\\midrule
\end{tabular}
\vspace*{-2em}
%\end{tabular}
\end{center}
\end{table}    

%\begin{table}[!th]
%\begin{center}
%%\begin{tabular}{p{18em}p{18em}}
%\vspace*{-2em}
%%\begin{tabular}{p{30em}}
%\caption{Regret Bound of Algorithms}
%\label{tab:comp-bds}
%%\begin{tabular}{p{5em}p{3em}p{7em}}
%\begin{tabular}{p{7 em}p{3em}p{7em}p{1em}p{1em}}
%\toprule
%Algorithm  &   \hspace*{1mm}Type & Gap-Independent & T & G \\
%\hline
%ImpCPD        & Active & $O\left(\sqrt{GT}\right)$ & Y & N\\
%UCB-CPD        & Active  & $O\left(\sqrt{GT}\log T\right)$ & N & N \\%\midrule
%CUSUM             & Active & $O\left( \sqrt{GT\log \frac{T}{G}}\right)$ & Y & Y \\%\midrule
%EXP3.R         & Active & $O\left( G\sqrt{T\log T}\right)$ & Y & N\\%\midrule
%DUCB        & Passive & $O\left(\sqrt{GT}\log T\right)$ & Y & Y\\
%SWUCB         & Passive & $O\left(\sqrt{GT\log T}\right)$ & Y & Y\\%\midrule
%Lower Bound         & N/A  & $\Omega\left( \sqrt{GT}\right)$ & Y & Y\\\midrule
%\end{tabular}
%\vspace*{-2em}
%%\end{tabular}
%\end{center}
%\end{table}    

%+ \dfrac{\alpha T}{K}
%$O\big(WG + \dfrac{T\log W}{W \Delta_{\min}^2} \big)$
%$O\big(WG + \dfrac{T\log W}{W \Delta_{\min}^2} \big)$
    %Also, our proposed algorithms do not require any additional exploration parameters to be tuned. Further, both of the proposed algorithms are anytime algorithm which does not require horizon $T$ as input. 
    
    The rest of the paper is organized as follows. We first state the notations, definitions, and assumptions required for this setting in Section~\ref{psbandit:notations}. Then we define our problem statement in Section~\ref{psbandit:probDef} and in Section~\ref{psbandit:algorithm} we present the changepoint detection algorithms. Section~\ref{psbandit:results} contains our main result, remarks and discussions, Section~\ref{psbandit:expt} contains numerical simulations where we test our proposed algorithms and finally we conclude in Section \ref{psbandit:conclusion}. The proofs are provided in Appendices.
    
    %and further discussions 
    %\ref{psbandit:appendix}
    %and in section~\ref{psbandit:related} we discuss the related works in this setting. We elaborate our contributions in section~\ref{psbandit:contribution} and 

==> probDef.tex <==
%Given the exploration-exploitation-changepoint dilemma, 
%in this setting
\vspace*{-0.3em}
\textbf{Regret Definition:} The objective of the learner is to minimize the cumulative regret till $T$, which is defined as, $R_{T}=\sum_{t'=1}^T \mu_{i^*_{t'}} - \sum_{t'=1}^T \mu_{ i_{t'}}  \indic{i_{t'}  \neq i^*_{t'} }$, 
%\vspace*{-0.6em}
%\begin{align*}
%R_{T}=\sum_{t'=1}^T \mu_{i^*_{t'}} - \sum_{t'=1}^T \mu_{ i_{t'}}  \indic{i_{t'}  \neq i^*_{t'} }
%\end{align*}
%\mu_{\mathbb{I}_{t'} = i \neq i^*_{t'}}
%\vspace*{-0.0 em}
where $T$ is the horizon, $\mu_{i^*_{t'}}$ is the expected mean of the optimal arm at the $t'$ timestep and $\mu_{ i_{t'}}  \indic{i_{t'}  \neq i^*_{t'} }$ is the expected mean of the arm chosen by the learner at the $t'$ timestep when it was not the optimal arm $i^*_{t'}$. The expected regret of an algorithm after $T$ rounds can be written as,
%Let $N_{i,g}$ is the number of times the learner has chosen arm $i_{}$ between $t_{g-1}$ to $t_{g}$.
%when it was not the optimal arm $i^*_{j}$
%$n_{i_{t'}\neq i^*_{t'},\forall t'=1:T}$
%\vspace*{-4em}
\vspace*{-0.8em}
\begin{align*}
\E[R_{T}] = \E\!\left[\sum_{t'=1}^T \mu_{i^*_{t'}} - \sum_{t'=1}^T \mu_{ i_{t'}}  \indic{i_{t'}  \neq i^*_{t'} }\right]
&\overset{(a)}{=} \!\!\E\left[\sum_{g=1}^{G}\sum_{t'=t_{g-1}}^{t_{g}} \!\mu_{i^*_{t'}} \! - \!  \sum_{g=1}^{G}\sum_{t'=t_{g-1}}^{t_{g}}  \!\mu_{ i_{t'}}  \indic{i_{t'}  \neq i^*_{t'} } \!\right]\\
%\begin{align*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\overset{(b)}{=}\sum_{g=1}^{G}\sum_{i = 1}^K\Delta^{opt}_{i,g}\E[N_{i,t_{g-1}:t_g}]
\end{align*}
%\mu_{\mathbb{I}_{t'} = i \neq i^*_{t'}}
%\vspace*{-4em}
where $(a)$ is from Assumption \ref{assm:global}, and $(b)$ from Definition \ref{Def:opt-gap}. 
%\indic{ i = i_{t'}}

\textbf{Problem Complexity:} We define the hardness of a changepoint $g\in\G$ using optimality and changepoint gaps by modifying the  definitions of \emph{problem complexity} as introduced in \cite{audibert2010best} for stochastic bandits,
%\begin{align*}
$\! H^{}_{1,g} \! = \!\max\!\left\lbrace\!\sum_{i=1}^{K}\!\frac{1}{(\Delta^{opt}_{i,g})^{2}}, \sum_{i\in\A^{chg}_g}^{}\!\frac{1}{(\Delta^{chg}_{i,g})^{2}}\! \right \rbrace\text{, } \hspace{0mm} H_{2,g} \!=\! \!\frac{\Delta^{opt}_{\max,g+1}}{\Delta(t_g,\delta)}$, 
%%%%%%%%%%%%%%%%%%%%%
%H^{}_{2,g} &=\max\left\lbrace\min_{i\in \mathcal{A}}\dfrac{i}{{(\Delta^{opt}_{(i),g})^{2}}}, \min_{i\in \mathcal{A}}\dfrac{i}{{(\Delta^{chg}_{(i),g})^{2}}} \right\rbrace
%\end{align*}
%where $(\Delta^{.}_{(i),g}: i\in\mathcal{A})$ is obtained by arranging $(\Delta^{.}_{i,g}:i\in\mathcal{A})$ in an increasing order. 
where $\Delta^{opt}_{\max,g+1}= \max_{i\in\A}\Delta^{opt}_{i,g+1}$. The hardness parameter $H_{2,g}$ captures the tradeoff between the minimum detectable gap $\Delta(t_g,\delta)$ and maximum optimality gap of the next changepoint $\Delta^{opt}_{\max,g+1}$ which serves as an upper bound to all such possible trade-offs at changepoint $g$. The relation between the above complexity terms can be derived as, 
%\begin{align*}
$H_{2,g}  \leq H^{}_{1,g} \leq \frac{K}{(\Delta(t_g,\delta))^2}(H_{2,g})$.
%H_{3,g} \leq H^{}_{2,g} \leq H^{}_{1,g}\leq \log(2K)H_{2,g}.
%\end{align*}
Note that, $\frac{\Delta^{opt}_{i,g}}{\Delta^{chg}_{i,g}} \leq H_{2,g}, \forall i\in\A^{chg}_g, g\in\G$. In the special case when $\Delta^{opt}_{i,g} = \Delta^{chg}_{i,g} = \Delta(t_g,\delta), \forall i\in\A_g^{chg}, g\in\G$, then,
%\begin{align*}
$H_{1,g} =  {K}{(\Delta(t_g,\delta))^{-2}},\text{ and } H_{2,g} = 1$.
%\end{align*}

 %and $H^{opt}_g = \frac{K}{(\Delta^{opt}_{\min})^2}$

% \ref{assm:space-gap}, and  \ref{assm:chg-gap}
%we substitute $\Delta^{opt}_{i,g}= \mu_{i^*,g}-\mu_{i,g}$

==> proofTheorem.tex <==
\subsubsection{Proof of Regret Bound of UCB-CPD}
\label{sec:proof:Theorem:1}


\begin{customproof}{1}
\label{proof:Lemma:1}
\label{proof:Theorem:1}
We start by noting that for any arm $i\in\A$, we detect a change-point if,
\begin{eqnarray}
&\hat{\mu}_{i,t_0:t'} - s_{i,t_0:t'} > \hat{\mu}_{i,t'+1:t} + s_{i,t'+1:t}, \text{ or }\nonumber\\ 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\hat{\mu}_{i,t_0:t'} +  s_{i,t_0:t'} < \hat{\mu}_{i,t'+1:t} - s_{i,t'+1:t}. \label{eq:CPD1}
\end{eqnarray}
 
where for any $t'\in[t_0,t]$ we define confidence interval term $s_{i,t_0:t'}$ for an arm $i\in\A$ at the $t$-th timestep as $s_{i,t_0:t'} = \sqrt{\dfrac{\log(\frac{t}{\sqrt{\delta}})}{n_{i,t_0:t'}}}$.
 
\textbf{Step 1.(Define Bad Event):} We define a bad event $\xi^{chg}_{i,t}$ for each arm $i\in\A$ as the complementary of events in Eq (\ref{eq:CPD1}) such that,
\begin{eqnarray}
\xi^{chg}_{i,t} = \bigg\lbrace\forall t'\in [t_0 , t]: \big(\hat{\mu}_{i,t_0:t'} - s_{i,t_0:t'} \leq \hat{\mu}_{i,t'+1:t} + s_{i,t'+1:t}\big) \bigcup \big(\hat{\mu}_{i,t_0:t'} +  s_{i,t_0:t'} \geq \hat{\mu}_{i,t'+1:t} - s_{i,t'+1:t}\big)\bigg\rbrace. \label{event:1}
\end{eqnarray}

\textbf{Step 2.(Define a stopping time):} We define a stopping time $\tau_{i,c_j}$ and $\tau'_{i,c_j}$ such that,

\begin{align*}
\tau_{i,c_j} = \min\left\lbrace t': s_{i,t_0:t'} < \dfrac{\Delta^{chg}_{i,c_j}}{2} \right\rbrace ,\hspace*{4em}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tau'_{i,c_j} = \min\left\lbrace t': s_{i,t'+1:t} < \dfrac{\Delta^{chg}_{i,c_j}}{2} \right\rbrace
\end{align*}


\textbf{Step 3.(Minimum pulls before $\tau_{i,c_j}$ and $\tau'_{i,c_j}$): } We define $n_{i,\min_{D}}$ as the minimum number of pulls  before $\tau_{i,c_j}$. Then, for $n_{i,t_0:\tau_{i,c_j}}\geq n_{i,\min_{D}} = \dfrac{4\log(\frac{t}{\sqrt{\delta}})}{(\Delta^{chg}_{i,c_j})^2}$ we can show that,

\begin{align*}
s_{i,t_0:\tau_{i,c_j}} = \sqrt{\dfrac{\log(\frac{t}{\sqrt{\delta}})}{n_{i,t_0:\tau_{i,c_j}}}} \leq \sqrt{\dfrac{\log(\frac{t}{\sqrt{\delta}})}{n_{i,\min_{D}}}} \leq \sqrt{\dfrac{(\Delta^{chg}_{i,c_j})^2\log(\frac{t}{\sqrt{\delta}})}{4\log(\frac{t}{\sqrt{\delta}})}} \leq \dfrac{\Delta^{chg}_{i,c_j}}{2}.
\end{align*} 

%so that the event $|\mu_{i,\rho_{c_{j-1}:c_j}}-\mu_{i,\rho_{c_j:c_{j+1}}}| < 2s_{i,t_0:\tau_{i,c_j}}$ never occurs and $|\mu_{i,\rho_{c_{j-1}:c_j}}-\mu_{i,\rho_{c_j:c_{j+1}}}|$ are sufficiently far apart.

\textbf{Step 4.(Bounding the probability of bad event): } In this step we bound the probability of the bad event $\xi^{chg}_{i,t}$ in Eq (\ref{event:1}). Now from Chernoff-Hoeffding inequality we know that for any constant $\epsilon > 0$,

\begin{align*}
\Pb\bigg\lbrace\left| \dfrac{\sum_{q=t_0}^{n} X_{i,q}}{n} - \mu_{i,t_0:n}\right| \geq \epsilon\bigg\rbrace \leq 2\exp\left(-2\epsilon^2 n\right)   
\end{align*}

Starting with the first condition of $\xi^{chg}_{i,t}$ and applying this inequality we can show that for a $\tau_{i,c_j}\in [t_0,t]$

\begin{align*}
\sum_{\tau_{i,c_j}=t_0}^{t} \sum_{q=t_0}^{\tau_{i,c_j}}\Pb\bigg\lbrace\hat{\mu}_{i,t_0:q} \leq \mu_{i,t_0:q} - s_{i,t_0:q}\bigg\rbrace \leq \sum_{\tau_{i,c_j}=t_0}^{t} \sum_{q=t_0}^{\tau_{i,c_j}}\exp\left(-2.\dfrac{\log(\frac{t}{\sqrt{\delta}})}{q}q \right)\leq \sum_{\tau_{i,c_j}=t_0}^{t} \sum_{q=t_0}^{\tau_{i,c_j}}\dfrac{\delta}{t^2}\leq \delta.
\end{align*}


%Summing over all $t'\in[t_0,t]$ we can show that,
%
%\begin{align*}
%\Pb\bigg\lbrace \hat{\mu}_{i,t_0:t'} \leq \mu_{i,t_0:t'} - s_{i,t_0:t'}\bigg\rbrace \leq \sum_{t'= t_0}^{t}\sum_{t'=\tau_{i,c_j}}^{t}\dfrac{\delta}{t^2}\leq \delta  
%\end{align*} 

%\begin{align*}
%\sum_{t'= t_0}^{t}\sum_{t'=\tau_{i,c_j}}^{t}\Pb\bigg\lbrace \hat{\mu}_{i,t_0:t'} \leq \mu_{i,\rho_{c_1:c_2}} - s_{i,t_0:t'}\bigg\rbrace &\leq \sum_{t'= t_0}^{t}\sum_{n_{i}=t_0}^{t'}\Pb\bigg\lbrace \hat{\mu}_{i,t_0:t'} \leq \mu_{i,t_0:t'} - s_{i,t_0:t'}\bigg\rbrace \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&\overset{(a)}{\leq} \sum_{t'= t_0}^{t}\sum_{n_{i}=t_0}^{t'}\exp\left( -2(s_{i,t_0:t'})^{2}t' \right)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&\leq \sum_{t'= t_0}^{t}\sum_{n_{i}=t_0}^{t'}\exp\left( -2\dfrac{\log(\frac{t}{\sqrt{\delta}})}{n_{i,t_0:t'}} t' \right)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&\leq \sum_{t'= t_0}^{t}\sum_{n_{i}=t_0}^{t'}\exp\left( -\dfrac{2\log(\frac{t}{\sqrt{\delta}})}{n_{i,t_0:t'}} t' \right)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&\overset{(b)}{\leq} \sum_{t'= t_0}^{t}\sum_{n_{i}=t_0}^{t'}\exp\left( -\dfrac{2\log(\frac{t}{\sqrt{\delta}})}{t'} t' \right)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&\leq \sum_{t'= t_0}^{t}\sum_{n_{i}=t_0}^{t'}\frac{\delta}{t^2}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&\leq \delta.
%\end{align*} 

%In the above formulation, $(a)$ is derived from the application of Chernoff-Hoeffding bound and for $(b)$ we apply the basic inequality that $n_{i,t_0:t'}\leq t', \forall t'\in [t_0,t]$.

Proceeding similarly as above, we can show that for a $\tau'_{i,c_j}\in[t_0,t]$,
\begin{align*}
\sum_{\tau'_{i,c_j}=t_0}^{t} \sum_{q=\tau'_{i,c_j}}^{t}\Pb\bigg\lbrace \hat{\mu}_{i,q:t} \geq \mu_{i,q:t} + s_{i,q:t}\bigg\rbrace \leq \sum_{\tau'_{i,c_j}=t_0}^{t} \sum_{q=\tau'_{i,c_j}}^{t}\dfrac{\delta}{t^2} \leq \delta.
\end{align*}

Summing the two up, the probability that the change-point for the arm $i$ is not detected by first condition of $\xi^{chg}_{i,t}$ for a $t'\in[t_0,t]$ is bounded by $\dfrac{2\delta}{t^2}$.

Again, for the second condition we can proceed in a similar way and show that for all $t'\in [t_0,t]$ and $\tau_{i,c_j},\tau'_{i,c_j}\in[t_0,t']$,
\begin{align*}
\Pb\bigg\lbrace\hat{\mu}_{i,t_0:t'} +  s_{i,t_0:t'} \geq \hat{\mu}_{i,t'+1:t} - s_{i,t'+1:t}\bigg\rbrace\leq \sum_{\tau_{i,c_j}=t_0}^{t} \sum_{q=t_0}^{\tau_{i,c_j}}\dfrac{\delta}{t^2} +\sum_{\tau'_{i,c_j}=t_0}^{t} \sum_{q=\tau'_{i,c_j}}^{t}\dfrac{\delta}{t^2} \leq 2\delta .
\end{align*} 

Hence, we can bound the probability of the bad event $\xi^{chg}_{i,t}$ for an arm $i\in\A$ by taking the union of all such events for all $t'\in[t_0,t]$ and for all $\tau_{i,c_j},\tau'_{i,c_j}\in[t_0,t']$ as,
\begin{align*}
\Pb\lbrace \xi^{chg}_{i,t}\rbrace \leq 4\delta.
\end{align*}

\end{customproof}



\begin{customproof}{2}
\label{proof:Theorem:1}

\textbf{Step 1.(Some notations and definitions):} Let, $n_{i,1:t}$ denote the number of times an arm $i\in\A$ is pulled  between $1$ to $t$-th timestep. We recall the definition of $\tau_{i,c_j}$, $\tau'_{i,c_j}$ for an arm $i$ and for a $t'\in[\tau_{i,c_{j-1}}, t]$ from Theorem \ref{Theorem:1} as,

\begin{align*}
\tau_{i,c_j} = \min\left\lbrace t': s_{i,\tau_{i,c_{j-1}}:t'} < \dfrac{\Delta^{chg}_{i,c_j}}{2} \right\rbrace ,\hspace*{4em}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tau'_{i,c_j} = \min\left\lbrace t': s_{i,t'+1:t} < \dfrac{\Delta^{chg}_{i,c_j}}{2} \right\rbrace
\end{align*}

We denote $n_{i,\min_{D}}= \dfrac{4\log(\frac{t}{\sqrt{\delta}})}{(\Delta^{chg}_{i,c_j})^2}$ as the minimum number of pulls required for an arm $i$ before $\tau_{i,c_j}$ or $\tau'_{i,c_j}$. We also recall the definition of the bad event $\xi^{chg}_{i,t}$ when the changepoint is not detected as,

\begin{align*}
\xi^{chg}_{i,t} = \bigg\lbrace\forall t'\in [\tau_{i,c_{j-1}} , t]:& \big(\hat{\mu}_{i,\tau_{i,c_{j-1}}:t'} - s_{i,\tau_{i,c_{j-1}}:t'} \leq \hat{\mu}_{i,t'+1:t} + s_{i,t'+1:t}\big) \\
%%%%%%%%%%%%%%%%%%
&\bigcup \big(\hat{\mu}_{i,\tau_{i,c_{j-1}}:t'} +  s_{i,\tau_{i,c_{j-1}}:t'} \geq \hat{\mu}_{i,t'+1:t} - s_{i,t'+1:t}\big)\bigg\rbrace.
\end{align*}


\textbf{Step 2.(Define an optimality stopping time): } We define an optimality stopping time $\tau^{opt}_{i,c_j}$ for a $\tau^{opt}_{i,c_j}\in[\tau_{i,c_{j-1}},t]$such that,

\begin{align*}
\tau^{opt}_{i,c_j} = \min\left\lbrace t: s'_{i,\tau_{i,c_{j-1}}:t} \leq \dfrac{\Delta^{opt}_{i,c_j}}{2} \right\rbrace
\end{align*}

where $s'_{i,\tau_{i,c_{j-1}}:t} = \sqrt{\dfrac{2\log(t)}{n_{i,\tau_{i,c_{j-1}}:t}}}$. 


\textbf{Step 3.(Minimum pulls of a sub-optimal arm): } We denote $n_{i,\min_{E}}$ as the minimum number of pulls required for a sub-optimal arm $i$ before $\tau^{opt}_{i,c_j}$ is satisfied. Indeed we can show that for $n_{i,\tau_{i,c_{j-1}}:t}\geq n_{i,\min_{E}} = \dfrac{8\log t}{(\Delta^{opt}_{i})^2}$,

\begin{align*}
s'_{i,\tau_{i,c_{j-1}}:t} = \sqrt{\dfrac{2\log(t)}{n_{i,\tau_{i,c_{j-1}}:t}}} \leq \sqrt{\dfrac{2\log(t)}{n_{i,\min_{E}}}}\leq \dfrac{\Delta^{opt}_{i,c_j}}{2}
\end{align*}

\textbf{Step 4.(Define the optimality bad event):} We define the optimality bad event $\xi^{opt}_{i,t}$ as,
%\begin{align*}
%\xi^{opt}_{i,t} = \left\lbrace\forall t'\in [\tau_{i,c_{j-1}} , t]: s'_{i,\tau_{i,c_{j-1}}:t'} > \dfrac{\Delta_{i,c_j}^{opt}}{2} \right\rbrace
%\end{align*}

\begin{align*}
\xi^{opt}_{i,t} = \left\lbrace\forall t'\in [\tau_{i,c_{j-1}} , t]: \hat{\mu}_{i^*} + s'_{i^*,\tau_{i,c_{j-1}},t} \leq  \hat{\mu}_{i} + s'_{i,\tau_{i,c_{j-1}},t} \right\rbrace
\end{align*}

For the above event to be true the following three events have to be true,

\begin{align*}
\xi^{opt}_{i,t} \subset \bigg\lbrace\forall t'\in [\tau_{i,c_{j-1}} , t]: &\lbrace\hat{\mu}_{i,\tau_{i,c_{j-1}}:t'} > \mu_{i,\tau_{i,c_{j-1}}:t'} + s'_{i,\tau_{i,c_{j-1}}:t'}\rbrace \\
%%%%%%%%%%%%%%%%%%%%%%
&\bigcup \lbrace\hat{\mu}_{i^*,\tau_{i,c_{j-1}}:t'} < \mu_{i^*,\tau_{i,c_{j-1}}:t'} - s'_{i^*,\tau_{i,c_{j-1}}:t'}\rbrace \\
%%%%%%%%%%%%%%%%%%%%%%
&\bigcup \lbrace (\mu_{i^*,\tau_{i^*,c_{j-1}}:t'} - \mu_{i,\tau_{i,c_{j-1}}:t'}) \leq 2s'_{i,\tau_{i,c_{j-1}}:t'} \rbrace\bigg\rbrace
\end{align*}

which implies that the sub-optimal arm $i$ has been over-estimated, the optimal arm $i^*$ has been under-estimated or there is sufficient gap between $(\mu_{i^*,\tau_{i^*,c_{j-1}}:t'} - \mu_{i,\tau_{i,c_{j-1}}:t'})$. But, from step $3$, we know that for $n_{i,\tau_{i,c_{j-1}}:t'}\geq n_{\min_E}$ the third event of $\xi^{opt}_{i,t}$ is not possible.

%\xi^{opt}_{i,t} = \left\lbrace\forall t'\in [\tau_{i,c_{j-1}} , t]: \hat{\mu}_{i,\tau_{i,c_{j-1}}:t'} - \mu_{i,\tau_{i,c_{j-1}}:t'} > 2s'_{i,\tau_{i,c_{j-1}}:t'}\right\rbrace

\textbf{Step 5.(Bound the number of pulls):} Let $\tau_{i,c_{0}}=1$ denoting the first timestep. Now, the total number of pulls  $n_{i,1:t}$ for an arm $i\in\A$ till $t$-th timestep is given by,

\begin{align*}
n_{i,1:t} &= \left[ 1 + \sum_{t'=K+1}^{t}\mathbf{1}_{\lbrace\mathbb{I}_{t'}=i\neq i^*_{t'}\rbrace} \right] \\
\end{align*}

We consider the contribution of each changepoint $c_{j}\in\G,\forall j=1,\ldots,G$ to the number of pulls $n_{i,1:t}$ and decompose the event $\lbrace\mathbb{I}_{t'}=i\neq i^*_{t'}\rbrace$ into four parts,

\begin{align*}
n_{i,1:t} &= \sum_{j=1}^{G}\bigg[ \underbrace{1 + \sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}\mathbf{1}_{\lbrace\mathbb{I}_{t'}=i\neq i^*_{t'},n_{i,\tau_{i,c_{j-1}}:t_{c_j}} < \max\lbrace n_{i,\min_E}, n_{i,\min_D}\rbrace\rbrace}}_{\textbf{part A}} + \underbrace{\sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}\mathbf{1}_{\lbrace\mathbb{I}_{t'}=i\neq i^*_{t'},n_{i,\tau_{i,c_{j-1}}:t_{c_j}} \geq \max\lbrace n_{i,\min_E}, n_{i,\min_D}\rbrace\rbrace}}_{\textbf{part B}}+\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\hspace*{-3em} \underbrace{\sum_{t'=t_{c_j}}^{\tau_{i,c_j}}\mathbf{1}_{\left\lbrace\mathbb{I}_{t'}=i\in\argmax_{i\in\A}\big\lbrace\argmax_{k\in\A}\lbrace \Delta^{opt}_{k,c_{j+1}}\rbrace \bigcup \argmin_{k\in\A}\lbrace \Delta^{chg}_{k,c_j}\rbrace \bigcup \argmax_{k\in\A}\lbrace \frac{\Delta^{opt}_{k,c_{j+1}}}{\Delta^{chg}_{k,c_j}} \rbrace\big\rbrace \right\rbrace}}_{\textbf{part C}} + \underbrace{\sum_{t'=t_{c_j}}^{\tau_{i,c_j}}\mathbf{1}_{\lbrace\mathbb{I}_{t'}=i\neq i^*_{t'},n_{i,t_{c_j}:\tau_{i,c_{j}}}\geq n_{i,\min_D}\rbrace}}_{\textbf{part D}} \bigg]
\end{align*}

where, \textbf{part A} refers to the minimum number of pulls required before either the expert discards the sub-optimal arm $i$ or a changepoint is detected between $\tau_{i,c_{j-1}}:t_{c_j}$, \textbf{part B} refers to the number of pulls due to bad event that the expert continues to pull the sub-optimal arm $i$ or the changepoint in not detected between $\tau_{i,c_{j-1}}:t_{c_j}$, \textbf{part C} refers to the pulls accrued due to the worst case events when the changepoint has occurred and has not been detected by the expert from $t_{c_j}:\tau_{i,c_{j}}$ and finally, \textbf{part D} refers to number of pulls for the bad event that the changepoint is not detected from $t_{c_j}:\tau_{i,c_{j}}$. 

Now, we will consider this parts individually and see their contribution to the number of pulls. For \textbf{part A},

\begin{align*}
\underbrace{1 + \sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}\mathbf{1}_{\lbrace\mathbb{I}_{t'}=i\neq i^*_{t'},n_{i,\tau_{i,c_{j-1}}:t_{c_j}} < \max\lbrace n_{i,\min_E}, n_{i,\min_D}\rbrace\rbrace}}_{\textbf{part A}} \leq 1 + n_{i,\min_E} + n_{i,\min_D} \overset{(a)}{=} 1 + \dfrac{8\log t}{(\Delta^{opt}_{i,c_{j-1}})^2} + \dfrac{4\log t}{(\Delta^{chg}_{i,c_{j-1}})^2}
\end{align*}

where $(a)$ is obtained from previous step $3,4$ and from step $3$ in Theorem \ref{Theorem:2}. Similarly, for \textbf{part B} we can show that the event,

\begin{align*}
\left\lbrace\mathbb{I}_{t'}=i\neq i^*_{t'},n_{i,\tau_{i,c_{j-1}}:t_{c_j}} \geq \max\lbrace n_{\min_E}, n_{i,\min_D}\rbrace\right\rbrace \subseteq \lbrace \xi^{opt}_{i,t_{c_j}} + \xi^{chg}_{i,t_{c_j}}  \rbrace
\end{align*}

which is obtained from step 4 and from Theorem \ref{Theorem:2}. Hence, we can upper bound \textbf{part B} as,

\begin{align*}
\underbrace{\sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}\mathbf{1}_{\lbrace\mathbb{I}_{t'}=i\neq i^*_{t'},n_{i,\tau_{i,c_{j-1}}:t_{c_j}} \geq \max\lbrace n_{i,\min_E}, n_{i,\min_D}\rbrace\rbrace}}_{\textbf{part B}} \leq \sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}\xi^{opt}_{i,t_{c_j}} + \sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}\xi^{chg}_{i,t_{c_j}}.
\end{align*}

Now, \textbf{part C} consist of the worst case scenario where the changepoint has occurred and has not been detected. A good learner always try to minimize the number of pulls that might occur in this period from $t_{c_j}:\tau_{i,c_j}$. Let the total number of pulls that might occur for this worst case scenario be denoted by $n_{i_{w},t_{c_j}:\tau_{i,c_j}}$ such that,

\begin{align*}
\underbrace{\sum_{t'=t_{c_j}}^{\tau_{i,c_j}}\mathbf{1}_{\left\lbrace\mathbb{I}_{t'}=i\in\argmax_{i\in\A}\big\lbrace\argmax_{k\in\A}\lbrace \Delta^{opt}_{k,c_{j+1}}\rbrace \bigcup \argmin_{k\in\A}\lbrace \Delta^{chg}_{k,c_j}\rbrace \bigcup \argmax_{k\in\A}\lbrace \frac{\Delta^{opt}_{k,c_{j+1}}}{\Delta^{chg}_{k,c_j}} \rbrace\big\rbrace \right\rbrace}}_{\textbf{part C}} = n_{i_{w},t_{c_j}:\tau_{i,c_j}}.
\end{align*}

Finally, for \textbf{part D} we can show that for $t'\in[t_{c_j}, \tau_{i,c_j}]$ or $t'\in[t_{c_j}, \tau'_{i,c_j}]$,
\begin{align*}
\left\lbrace\mathbb{I}_{t'}=i\neq i^*_{t'},n_{i,t_{c_j}:\tau_{i,c_{j}}}\geq  n_{\min_D}\right\rbrace \subseteq \lbrace \xi^{chg}_{i,\tau_{i,c_j}}  \rbrace \bigcup \lbrace (\mu_{i^*,t_{c_j}:\tau_{i^*,c_{j}}} - \mu_{i,t_{c_j}:\tau_{i^*,c_{j}}}) < 2s_{i,t_{c_j}:\tau_{i^*,c_{j}}} \rbrace.
\end{align*}

But from step 5 in Theorem \ref{Theorem:2} we know that for $n_{i,\tau_{c_{j-1}}:\tau_{c_{j}}}\geq n_{i,\min_D}$ then the event $ (\mu_{i,t_{c_j}:\tau_{i,c_{j}}} - \mu_{i,t_{c_j}:\tau_{i,c_{j}}}) < 2s_{i,t_{c_j}:\tau_{i,c_{j}}}$ is not possible. Hence, we can show that \textbf{part D} is upper bounded by,

\begin{align*}
\underbrace{\sum_{t'=t_{c_j}}^{\tau_{i,c_j}}\mathbf{1}_{\lbrace\mathbb{I}_{t'}=i\neq i^*_{t'},n_{i,t_{c_j}:\tau_{i,c_{j}}}\geq n_{i,\min_D}\rbrace}}_{\textbf{part D}} \leq n_{i,\min_D} + \sum_{t'=t_{c_j}}^{\tau_{i,c_j}}\xi^{chg}_{i,\tau_{i,c_j}} \leq n_{i,\min_D} + \sum_{t'=\tau_{i,c_{j-1}}}^{\tau_{i,c_j}}\xi^{chg}_{i,\tau_{i,c_j}} = \dfrac{4\log t}{(\Delta^{chg}_{i,c_{j}})^2} + \sum_{t'=\tau_{i,c_{j-1}}}^{\tau_{i,c_j}}\xi^{chg}_{i,\tau_{i,c_j}}.
\end{align*}


%\begin{align*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&\overset{(a)}{\leq} \sum_{j=1}^{G}\bigg[ 1 + \max\lbrace n_{i,\min_E}, n_{i,\min_D}\rbrace + \sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}\mathbf{1}_{\lbrace\mathbb{I}_{t'}=i\neq i^*_{t'},n_{i,\tau_{i,c_{j-1}}:t_{c_j}} \geq \max\lbrace n_{i,\min_E}, n_{i,\min_D}\rbrace\rbrace}+\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&\hspace*{-3em} \sum_{t'=t_{c_j}}^{\tau_{i,c_j}}\mathbf{1}_{\left\lbrace\mathbb{I}_{t'}=i\in\argmax_{i\in\A}\big\lbrace\argmax_{k\in\A}\lbrace \Delta^{opt}_{k,c_{j+1}}\rbrace \bigcup \argmin_{k\in\A}\lbrace \Delta^{chg}_{k,c_j}\rbrace \bigcup \argmax_{k\in\A}\lbrace \frac{\Delta^{opt}_{k,c_{j+1}}}{\Delta^{chg}_{k,c_j}} \rbrace\big\rbrace \right\rbrace} + \sum_{t'=t_{c_j}}^{\tau_{i,c_j}}\mathbf{1}_{\lbrace\mathbb{I}_{t'}=i\neq i^*_{t'},n_{i,t_{c_j}:\tau_{i,c_{j}}}\geq n_{i,\min_D}\rbrace} \bigg]\\
%\end{align*}
%
%Now, combining the result of step 4 and from Theorem \ref{Theorem:2} we can show that,
%\begin{align*}
%\mathbb{I}_{t'}=i\neq i^*_{t'},n_{i,\tau_{i,c_{j-1}}:t_{c_j}} \geq \max\lbrace n_{\min_E}, n_{i,\min_D}\rbrace \subseteq \lbrace \xi^{opt}_{i,t_{c_j}} + \xi^{chg}_{i,t_{c_j}}  \rbrace
%\end{align*}
%
%Similarly, we can show that for $t'\in[t_{c_j}, \tau_{i,c_j}]$ or $t'\in[t_{c_j}, \tau'_{i,c_j}]$,
%\begin{align*}
%\mathbb{I}_{t'}=i\neq i^*_{t'},n_{i,t_{c_j}:\tau_{i,c_{j}}}\geq  n_{\min_D} \subseteq \lbrace \xi^{chg}_{i,\tau_{i,c_j}}  \rbrace \bigcup \lbrace (\mu_{i^*,t_{c_j}:\tau_{i^*,c_{j}}} - \mu_{i,t_{c_j}:\tau_{i^*,c_{j}}}) < 2s_{i,t_{c_j}:\tau_{i^*,c_{j}}} \rbrace.
%\end{align*}
%
%But from step 5 in Theorem \ref{Theorem:2} we know that for $n_{i,\tau_{c_{j-1}}:\tau_{c_{j}}}\geq n_{i,\min_D}$ then the event $ (\mu_{i,t_{c_j}:\tau_{i,c_{j}}} - \mu_{i,t_{c_j}:\tau_{i,c_{j}}}) < 2s_{i,t_{c_j}:\tau_{i,c_{j}}}$ is not possible. Hence, we get,
%
%\begin{align*}
%n_{i,1:t} &= \left[ 1 + \sum_{t'=K+1}^{t}\mathbf{1}_{\lbrace\mathbb{I}_{t'}=i\neq i^*_{t'}\rbrace} \right] \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&= \sum_{j=1}^{G}\bigg[ 1 + \max\lbrace n_{i,\min_E}, n_{i,\min_D}\rbrace + \sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}\mathbf{1}_{\lbrace\mathbb{I}_{t'}=i_{t'}\neq i^*_{t'},n_{i,\tau_{i,c_{j-1}}:t_{c_j}} \geq \max\lbrace n_{i,\min_E}, n_{i,\min_D}\rbrace\rbrace} + \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&\hspace*{-3em}\sum_{t'=t_{c_j}}^{\tau_{i,c_j}}\mathbf{1}_{\left\lbrace\mathbb{I}_{t'}=i\in\argmax_{i\in\A}\big\lbrace\argmax_{k\in\A}\lbrace \Delta^{opt}_{k,c_{j+1}}\rbrace \bigcup \argmin_{k\in\A}\lbrace \Delta^{chg}_{k,c_j}\rbrace \bigcup \argmax_{k\in\A}\lbrace \frac{\Delta^{opt}_{k,c_{j+1}}}{\Delta^{chg}_{k,c_j}} \rbrace\big\rbrace \right\rbrace} + \sum_{t'=t_{c_j}}^{\tau_{i,c_j}}\mathbf{1}_{\lbrace\mathbb{I}_{t'}=i\neq i^*_{t'},n_{i,t_{c_j}:\tau_{i,c_{j}}}\geq n_{i,\min_D}\rbrace} \bigg]\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&\leq \sum_{j=1}^{G}\bigg[\underbrace{1 + n_{i,\min_E} + \sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}\mathbf{1}_{\xi^{opt}_{i,t_{c_j}}}}_{\textbf{optimality detection from $\tau_{i,c_{j-1}}:t_{c_j}$}} + \underbrace{n_{i,\min_D} +\sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}\mathbf{1}_{\xi^{chg}_{i,t_{c_j}}}}_{\textbf{changepoint detection from $\tau_{i,c_{j-1}}:t_{c_j}$}}
%\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%& +\underbrace{\sum_{t'=t_{c_j}}^{\tau_{i,c_j}}\mathbf{1}_{\left\lbrace\mathbb{I}_{t'}=i\in\argmax_{i\in\A}\big\lbrace\argmax_{k\in\A}\lbrace \Delta^{opt}_{k,c_{j+1}}\rbrace \bigcup \argmin_{k\in\A}\lbrace \Delta^{chg}_{k,c_j}\rbrace \bigcup \argmax_{k\in\A}\lbrace \frac{\Delta^{opt}_{k,c_{j+1}}}{\Delta^{chg}_{k,c_j}} \rbrace\big\rbrace \right\rbrace}}_{\textbf{pull arm for worst case event from $t_{c_j}:\tau_{i,c_j}$}} + \underbrace{n_{i,\min_D} +\sum_{t'=t_{c_j}}^{\tau_{i,c_{j}}}\mathbf{1}_{\xi^{chg}_{i,\tau_{i,c_j}}}}_{\textbf{changepoint detection from $t_{c_j}:\tau_{i,c_{j}}$}}\bigg] 
%\end{align*}


%\begin{align*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%& = \sum_{j=1}^{G}\bigg[ 1 + \underbrace{\sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}\mathbb{I}\left({s'_{i,\tau_{i,c_{j-1}}:t'} \leq \dfrac{\Delta^{opt}_{i,c_j}}{2}}\right) +  \sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}\mathbb{I}\left(s'_{i,\tau_{i,c_{j-1}}:t'} > \dfrac{\Delta^{opt}_{i,c_j}}{2}\right)}_{\textbf{optimality detection till $\tau_{i,c_{j-1}}:t_{c_j}$}} + \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%& \underbrace{\sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}\mathbb{I}\left({s_{i,\tau_{i,c_{j-1}}:t'} \leq \dfrac{\Delta^{chg}_{i,c_j}}{2} }\right) +  \sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}\mathbb{I}\left({s_{i,\tau_{i,c_{j-1}}:t'} > \dfrac{\Delta^{chg}_{i,c_j}}{2} }\right)}_{\textbf{changepoint detection till $\tau_{i,c_{j-1}}:t_{c_j}$}} + \underbrace{\mathbb{I}\left( i_{t_{c_j:\tau_{i,c_j}}}=\max\lbrace \Delta^{opt}_{i,c_j},\forall i\in\A \rbrace\right)}_{\textbf{pull arm with $\max_{i\in\A}\lbrace \Delta^{opt}_{i,c_{j}} \rbrace$ till $t_{c_j}:\tau_{i,c_j}$}} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%& + \underbrace{\sum_{t'=t_{c_j}}^{\tau_{i,c_j}}\mathbb{I}\left({s_{i,\tau_{i,c_{j-1}}:t'} \leq \dfrac{\Delta^{chg}_{i,c_j}}{2} }\right) +  \sum_{t'=t_{c_j}}^{\tau_{i,c_j}}\mathbb{I}\left({s_{i,\tau_{i,c_{j-1}}:t'} > \dfrac{\Delta^{chg}_{i,c_j}}{2} }\right)}_{\textbf{changepoint detection till $t_{c_j}:\tau_{i,c_j}$}} \bigg]\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\end{align*}

\textbf{Step 6.(Bound the expected regret):} Now, taking expectation over $n_{i,1:t}$, and considering the contributions form $\textbf{parts A, B, C, D}$ we can show that,

\begin{align*}
\E[n_{i,1:t}] &\leq \sum_{j=1}^{G}\bigg[ \underbrace{1 + n_{i,\min_{E}} +  \sum_{t'=n_{i,\min_{E}}}^{t_{c_j}}\Pb\lbrace \xi^{opt}_{i,t_{c_j}} \rbrace}_{\textbf{A1) expected pulls from $\tau_{i,c_{j-1}}:t_{c_j}$ for optimality detection}} + \underbrace{n_{i,\min_{D}}  +  \sum_{t'=n_{i,\min_{D}}}^{t_{c_j}}\Pb\lbrace \xi^{chg}_{i,t_{c_j}}\rbrace}_{\textbf{B1) expected pulls from $\tau_{i,c_{j-1}}:t_{c_j}$ for changepoint detection}}  \\
%%%%%%%%%%%%%%%%%%%%%%%%%
 &+ \underbrace{n_{i_{w},t_{c_j}:\tau_{i,c_j}}}_{\textbf{C1) worst case expected pulls from $t_{c_j}:\tau_{i,c_j}$}} + \underbrace{ n_{i,\min_{D}} + \sum_{t'=n_{i,\min_{D}}}^{\tau_{i,c_j}}\Pb\lbrace \xi^{chg}_{i,\tau_{i,c_j}}\rbrace}_{\textbf{D1) expected pulls from $t_{c_j}:\tau_{i,c_{j}}$ for changepoint detection}} \bigg]\\
%%%%%%%%%%%%%%%%%%%%%%%%%
\end{align*}

%where, $n_{i_{w},t_{c_j}:\tau_{i,c_j}}$ denotes the number of times arm(s) are pulled for the worst case event,
%\begin{align*}
%\sum_{t'=t_{c_j}}^{\tau_{i,c_j}}\mathbf{1}_{\left\lbrace\mathbb{I}_{t'}=i\in\argmax_{i\in\A}\big\lbrace\argmax_{k\in\A}\lbrace \Delta^{opt}_{k,c_{j+1}}\rbrace \bigcup \argmin_{k\in\A}\lbrace \Delta^{chg}_{k,c_j}\rbrace \bigcup \argmax_{k\in\A}\lbrace \frac{\Delta^{opt}_{k,c_{j+1}}}{\Delta^{chg}_{k,c_j}} \rbrace\big\rbrace \right\rbrace}.
%\end{align*}
Now, for \textbf{part A1} we obtain from from Theorem 1 in \citet{auer2002finite} that,

\begin{align*}
\sum_{t'=n_{i,\min_{E}}}^{t_{c_j}}\Pb\lbrace \xi^{opt}_{i,t_{c_j}} \rbrace &\leq \sum_{t'=1}^{\infty}\sum_{n_{i}=n_{\min_{E}}}^{t'}\sum_{n_{i^*}=1}^{t'}\left\lbrace \Pb\left(\hat{\mu}_{i} \geq \mu_{i} + \dfrac{2\log(t)}{n_i}\right) + \Pb\left(\hat{\mu}_{i^*} \leq \mu_{i^*}- \dfrac{2\log(t)}{n_{i^*}}\right)\right\rbrace\\
&\overset{(a)}{\leq} \sum_{t'=1}^{\infty}\sum_{n_{i}=1}^{t'}\sum_{n_{i^*}=1}^{t'}\dfrac{2}{(t')^4} \leq \dfrac{\pi^2}{3}.
\end{align*}

where, $(a)$ comes from the application of Chernoff-Hoeffding bound. Again, for \textbf{part C1} we use the assumption \ref{assm:space-gap}, assumption \ref{assm:chg-gap} and discussion \ref{dis:gap-delay} to upper bound it as,

\begin{align*}
\underbrace{n_{i_{w},t_{c_j}:\tau_{i,c_j}}}_{\textbf{C1) worst case expected pulls from $t_{c_j}:\tau_{i,c_j}$}} \leq \dfrac{4\log(t\sqrt{t})}{(\Delta^{chg}_{\epsilon_0,c_j})^{2}}.
\end{align*}

Substituting these in $\E[n_{i,1:t}]$ we get,

\begin{align*}
\E[n_{i,1:t}] &\overset{(a)}{\leq} \sum_{j=1}^{G}\bigg[\underbrace{1+ \dfrac{8\log t}{(\Delta^{opt}_{i,c_j})^2} + \dfrac{\pi^2}{3}}_{\textbf{part A1}} + \underbrace{\dfrac{4\log(\frac{t}{\sqrt{\delta}})}{(\Delta^{chg}_{i,c_j})^2} + \sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}4\delta}_{\textbf{part B1}} + \underbrace{\dfrac{4\log(t\sqrt{t})}{(\Delta^{chg}_{\epsilon_0,c_j})^{2}}}_{\textbf{part C1}}
%%%%%%%%%%%%%%%%%%
+ \underbrace{\dfrac{4\log(\frac{t}{\sqrt{\delta}})}{(\Delta^{chg}_{i,c_j})^2} + \sum_{t'=\tau_{i,c_{j-1}}+K+1}^{\tau_{i,c_j}}4\delta}_{\textbf{part D1}} \bigg]\\
%%%%%%%%%%%%%%%%%%%%%%%%%
&\overset{(b)}{\leq} \sum_{j=1}^{G}\left[1+ \dfrac{8\log t}{(\Delta^{opt}_{i,c_j})^2} + \dfrac{\pi^2}{3} + \dfrac{4\log(t\sqrt{t})}{(\Delta^{chg}_{i,c_j})^2} + \sum_{t'=\tau_{i,c_{j-1}}+K+1}^{t_{c_j}}\dfrac{4}{t} + \dfrac{4\log(t\sqrt{t})}{(\Delta^{chg}_{\epsilon_0,c_j})^{2}} +\dfrac{4\log(t\sqrt{t})}{(\Delta^{chg}_{i,c_j})^2} + \sum_{t'=\tau_{i,c_{j-1}}+K+1}^{\tau_{i,c_j}}\dfrac{4}{t} \right]\\
\end{align*}

where, $(a)$ comes from the result of Theorem \ref{Theorem:1} and in $(b)$ we substitute $\delta=\dfrac{1}{t}$ from Remark \ref{Rem:1}.

%\max_{i\in\A}\left\lbrace \dfrac{\Delta^{opt}_{i,c_j}}{\Delta^{chg}_{i,c_j}}\right\rbrace
%Hence, combining the two above we can show that,
%
%\begin{align*}
%& n_{i\neq i^*_{t'} ,\forall t'\in[t_0:t]} = \sum_{j=1}^{G}\bigg\lbrace\mathbb{I}_{\text{Expert Algorithm from $t_0:t_{c_j}$}} + \mathbb{I}_{i,t_{c_j}:\tau_{i,c_j}}\bigg\rbrace \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&= \sum_{j=1}^{G}\bigg\lbrace n_{i,\min_{Expert}} + \sum_{t'= t_0+K+1}^{t_{c_j}}\big\lbrace\min\hat{\mu}_{i^*,t_0:t'} + s'_{i^*,t_0:t'} < \max\hat{\mu}_{i,t_0:t'} + s'_{i,t_0:t'}, n_{i,t_0:t'}\geq n_{i,\min_{Expert}} \big\rbrace + \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&  n_{i,\min_{Detect}} + \sum_{t'= t_0}^{\tau_{i,c_j}}\big\lbrace \big(\hat{\mu}_{i,t_0:t'} - s_{i,t_0:t'} \geq \hat{\mu}_{i,t':t_{c_j}} + s_{i,t':t_{c_j}}\big) \bigcup \big( \hat{\mu}_{i,t_0:t'} +  s_{i,t_0:t'} < \hat{\mu}_{i,t'+1:t_{c_j}} - s_{i,t'+1:t_{c_j}}\big), n_{i,t_0:t'}\geq n_{i,\min_{Detect}}  \big\rbrace \bigg\rbrace \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&\leq  \sum_{j=1}^{G} \bigg\lbrace n_{i,\min_{Expert}} + \sum_{t'=t_0}^{\infty}\sum_{n_{i^*,t_0:t'}=t_0}^{t'}\sum_{n_{i,t_0:t'}=n_{i,\min_{Expert}}}^{t'}\big\lbrace  \hat{\mu}_{i,t_0:t'} +  s'_{i,t_0:t'} < \hat{\mu}_{i,t'+1:t_{c_j}} - s'_{i,t'+1:t_{c_j}} \big\rbrace + \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%& n_{i,\min_{Detect}} + \sum_{t'= t_0}^{\tau_{i,c_j}}\big\lbrace \big(\hat{\mu}_{i,t_0:t'} - s_{i,t_0:t'} \geq \hat{\mu}_{i,t':t_{c_j}} + s_{i,t':t_{c_j}}\big) \bigcup \big( \hat{\mu}_{i,t_0:t'} +  s_{i,t_0:t'} < \hat{\mu}_{i,t'+1:t_{c_j}} - s_{i,t'+1:t_{c_j}}\big), n_{i,t_0:t'}\geq n_{i,\min_{Detect}}  \big\rbrace\bigg\rbrace \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\end{align*}
%
%Now, taking expectation on both sides we can show that $\E[n_{i\neq i^*_{t'} ,\forall t'\in[t_0:t]}]$ is bounded by,
%
%\begin{eqnarray}
%%&\E[n_{i\neq i^*_{t'} ,\forall t'\in[t_0:t]}] \nonumber \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%& \sum_{j=1}^{G} \bigg\lbrace n_{i,\min_{Expert}} + \sum_{t'=t_0}^{\infty}\sum_{n_{i^*,t_0:t'}=t_0}^{t'}\sum_{n_{i,t_0:t'}=n_{i,\min_{Expert}}}^{t'}\Pb\big\lbrace  \hat{\mu}_{i^*,t_0:t'} +  s'_{i^*,t_0:t'}\big\rbrace  + \Pb\big\lbrace \hat{\mu}_{i,t'+1:t_{c_j}} - s'_{i,t'+1:t_{c_j}} \big\rbrace \nonumber \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&  + n_{i,\min_{Detect}} + \sum_{t'= t_0}^{\tau_{i,c_j}}\big\lbrace \Pb\big(\hat{\mu}_{i,t_0:t'} - s_{i,t_0:t'} \geq \hat{\mu}_{i,t'+1:t_{c_j}} + s_{i,t'+1:t_{c_j}}\big) + \Pb\big( \hat{\mu}_{i,t_0:t'} +  s_{i,t_0:t'} < \hat{\mu}_{i,t'+1:t_{c_j}} - s_{i,t'+1:t_{c_j}}\big) \big\rbrace \bigg\rbrace \label{eq:Reg2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\end{eqnarray}
%
%For the first term in Eq $(\ref{eq:Reg2})$, considering the single expert is running the UCB1 algorithm, it can be bounded by using Theorem 1 of \citet{auer2002finite} and the second term in Eq $(\ref{eq:Reg2})$, considering the result of Theorem \ref{Theorem:1} and Remark \ref{Rem:1}, it can be bounded by,
%
%\begin{align*}
%& \E[n_{i\neq i^*_{t'} ,\forall t'\in[t_0:t]}] \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&= \sum_{j=1}^{G} \bigg\lbrace n_{i,\min_{Expert}} + \sum_{t'=t_0}^{\infty}\sum_{n_{i^*,t_0:t'}=t_0}^{t'}\sum_{n_{i,t_0:t'}=n_{i,\min_{Expert}}}^{t'}\big\lbrace \Pb\lbrace\hat{\mu}_{i^*,t_0:t'} \leq {\mu}_{i^*,t_0:t'} -  s'_{i^*,t_0:t'}\rbrace + \Pb\lbrace\hat{\mu}_{i,t':t_{c_j}} \geq {\mu}_{i,t'+1:t_{c_j}} + s'_{i,t'+1:t_{c_j}}\rbrace \big\rbrace +\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%& n_{i,\min_{Detect}} + \sum_{t'= t_0}^{\tau_{i,c_j}}\big\lbrace \Pb\big(\hat{\mu}_{i,t_0:t'} - s_{i,t_0:t'} \geq \hat{\mu}_{i,t':t_{c_j}} + s_{i,t':t_{c_j}}\big) + \Pb\big( \hat{\mu}_{i,t_0:t'} +  s_{i,t_0:t'} < \hat{\mu}_{i,t'+1:t_{c_j}} - s_{i,t'+1:t_{c_j}}\big) \big\rbrace \bigg\rbrace \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%&\leq \sum_{j=1}^{G} \bigg\lbrace \dfrac{8\log(t)}{\Delta_{i,c_j}'^{2}} + 1 + \dfrac{\pi^2}{3} + \dfrac{4\log(t\sqrt{t})}{\Delta_{i,c_j}^{2}} + \dfrac{4}{t} \bigg\rbrace\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\end{align*}

Hence, the regret upper bound is given by summing over all arms in $\A$,

\begin{align*}
\E[R_t] &\leq \sum_{i=1}^{K}\sum_{j=1}^{G}\E[n_{i_{t'}\neq i^*_{t'} ,\forall t'\in[t_{c_{j-1}}:t_{c_j}]}]\Delta^{opt}_{i,c_j} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\leq \sum_{i=1}^{K}\sum_{j=1}^{G} \bigg\lbrace 1 + \dfrac{8\log(t)}{\Delta^{opt}_{i,c_j}} + \dfrac{\pi^2}{3} + n_{i_w,t_{c_j}:\tau_{i_w,c_j}} + \dfrac{4\Delta^{opt}_{i,c_{j}}\log(t\sqrt{t})}{(\Delta^{chg}_{i,c_j})^2} +\dfrac{4\Delta^{opt}_{i,c_{j+1}}\log(t\sqrt{t})}{(\Delta^{chg}_{i,c_j})^{2}} + 8 \bigg\rbrace\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& \overset{(a)}{\leq} \sum_{i=1}^{K}\sum_{j=1}^{G} \bigg\lbrace 9 + \dfrac{8\log(t)}{\Delta^{opt}_{i,c_j}} + \dfrac{\pi^2}{3} + \dfrac{4\Delta^{opt}_{\max,c_{j+1}}\log(t\sqrt{t})}{(\Delta^{chg}_{\epsilon_0,c_j})^{2}} + \dfrac{4\Delta^{opt}_{i,c_{j}}\log(t\sqrt{t})}{(\Delta^{chg}_{i,c_j})^2} + \dfrac{4\Delta^{opt}_{i,c_{j+1}}\log(t\sqrt{t})}{(\Delta^{chg}_{i,c_j})^{2}}\bigg\rbrace
\end{align*}

where, $(a)$ is obtained from assumption \ref{Def:e-chg-gap}.
\end{customproof}

\subsubsection{Proof of Regret Bound of ImpCPD}
\label{sec:proof:Theorem:2}


\begin{customproof}{3}
\label{proof:Theorem:2}

We proceed as like Theorem 3.1 in \citet{auer2010ucb} and we combine the changepoint detection sub-routine with this. 

\textbf{Step 0.(Vital Assumption for proving):} In this proof, we assume that all the changepoints are detected by the algorithm with some delay. Since, all the gaps are significant (Assumption \ref{assm:chg-gap}) and there is sufficient delay between two changepoints (Assumption \ref{assm:space-gap}), we can take this assumption for proving the result.

\textbf{Step 1.(Define some notations):} In this proof, we define the confidence interval for the $i$-th arm as $s_i=\sqrt{\dfrac{\alpha\log(\psi T\epsilon_m^2)}{n_{i}}}$. The phase numbers are denoted by $m=0,1,\ldots,M$ where $M=\frac{1}{2}\log_{1+\gamma}\frac{T}{e}$. For the sake of brevity, in this proof we write $n_i$ instead of $n_{i,t_0:t_p}$ denoting the number of times the arm $i$ is pulled between two restarts, ie, between $t_0$ to $t_p$ (as shown in algorithm). For each sub-optimal arm $i$, we consider their contribution to cumulative regret individually till each of the changepoint is detected. We also define $\A'=\left\lbrace i\in\A: \Delta^{opt}_{i,c_j}\geq \sqrt{\frac{e}{T}}, \Delta^{chg}_{i,c_j}\geq \sqrt{\frac{e}{T}},\forall c_j\in\G \right\rbrace$.

\textbf{Step 2.(Define an optimality stopping phase $m_{i,c_j}$):} We define an optimality stopping phase $m_{i,c_j}$ for a sub-optimal arm $i\in\A'$ as the first phase after which the arm $i$ is no longer pulled till the $c_j$-th changepoint is detected such that for $0<\gamma\leq 1$,

\begin{align*}
m_{i,c_j} = \min\left\lbrace m: \sqrt{\alpha\epsilon_{m}} < \dfrac{\Delta^{opt}_{i,c_j}}{2(1+\gamma)^2} \right\rbrace
\end{align*} 

\textbf{Step 3.(Define a changepoint stopping phase $p_{i,c_j}$):} We define a changepoint stopping phase $p_{i,c_j}$ for an arm $i\in\A'$ such that it is the first phase when the changepoint $c_j$ is detected such that for $0<\gamma\leq 1$,

\begin{align*}
p_{i,c_j} = \min\left\lbrace m: \sqrt{\alpha\epsilon_{m}} < \dfrac{\Delta^{chg}_{i,c_j}}{2(1+\gamma)^2} \right\rbrace
\end{align*}

\textbf{Step 4.(Regret for sub-optimal arm $i$ being pulled after $m_{i,c_j}$-th phase):} Note, that on or after the $m_{i,c_j}$-th phase a sub-optimal arm $i\in\A'$ is not pulled anymore if these four conditions hold,

\begin{eqnarray}
\hat{r}_{i,c_j} < r_{i,c_j} + s_i, \hspace*{2em}  \hat{r}_{i*,c_j} > r_{i*,c_j} - s_{i*}, \hspace*{2em} s_i > s_{i*}, \hspace*{2em} n_i < n_{i*} \label{eq:arm-pull-opt}
\end{eqnarray}

Also, in the $m_{i,c_j}$-th phase if $n_i \geq \ell_{m_{i,c_j}} = \dfrac{\log(\psi T\epsilon_{m_{i,c_j}}^2)}{2\epsilon_{m_{i,c_j}}}$ then we can show that,
\begin{align*}
s_i = \sqrt{\dfrac{\alpha\log(\psi T\epsilon_{m_{i,c_j}}^2)}{2n_{i}}} \leq \sqrt{\dfrac{\alpha\log(\psi T\epsilon_{m_{i,c_j}}^2)}{2\ell_{m_{i,c_j}}}} \leq \sqrt{\alpha\epsilon_{m_{i,c_j}}\dfrac{\log(\psi T\epsilon_{m_{i,c_j}}^2)}{\log(\psi T\epsilon_{m_{i,c_j}}^2)}} \leq \dfrac{\Delta^{opt}_{i,c_j}}{2(1+\gamma)^2}.
\end{align*}

If indeed the four conditions in equation \ref{eq:arm-pull-opt} hold then we can show that in the $m_{i,c_j}$-th phase,

\begin{align*}
\hat{r}_{i,c_j} + s_i \leq {r}_{i,c_j} + 2(1+\gamma)^2 s_i - (1+\gamma)^2s_i \leq {r}_{i,c_j} + \Delta^{opt}_{i,c_j} - (1+\gamma)^2s_i \leq {r}_{i*,c_j} - (1+\gamma)^2s_{i*} \leq \hat{r}_{i*,c_j} - s_{i*}
\end{align*}

Hence, the sub-optimal arm $i$ is no longer pulled on or after the $m_{i,c_j}$-th phase. Therefore, to bound the number of pulls of the sub-optimal arm $i$, we need to bound the probability of the complementary of the four events in equation \ref{eq:arm-pull-chg}.

For the first event in equation \ref{eq:arm-pull-opt}, using Chernoff-Hoeffding bound we can bound the probability of the complementary of that event by,

\begin{align*}
&\sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\Pb\lbrace \hat{r}_{i,c_j} \geq  r_{i,c_j} + s_i \rbrace \leq \sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\exp\left(-2s_i^2n_i \right)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\leq \sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\exp\left(-2\dfrac{\alpha\log(\psi T\epsilon_{m_{}}^2)}{2n_i}n_i \right)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\leq \sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\dfrac{1}{\psi T\epsilon_{m_{}}^2} \leq \sum_{m=0}^{m_{i,c_j}}\dfrac{\log(\psi T\epsilon_{m_{}}^2)}{2\epsilon_{m_{}}}\dfrac{1}{(\psi T\epsilon_{m_{}}^2)^{\alpha}} \leq  \dfrac{\log(\psi T  \epsilon_{m_{i,c_j}}^2)}{2(\psi T)^{\alpha}}\sum_{m=0}^{m_{i,c_j}}\dfrac{1}{\epsilon_{m_{}}^{2\alpha +1}}.
\end{align*}

Similarly, for the second event in equation \ref{eq:arm-pull-opt}, we can bound the probability of its complementary event by,

\begin{align*}
\sum_{m=0}^{m_{i,c_j}}\sum_{n_{i*} =1}^{\ell_{m_{}}}\Pb\lbrace \hat{r}_{i*,c_j} \leq  r_{i*,c_j} - s_{i*} \rbrace &\leq \sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\exp\left(-2(s_{i*})^2n_{i*} \right)\leq \dfrac{\log(\psi T \epsilon_{m_{i,c_j}}^2)}{2(\psi T)^{\alpha}}\sum_{m=0}^{m_{i,c_j}}\dfrac{1}{\epsilon_{m_{}}^{2\alpha +1}}.
\end{align*}


Also, for the third event in equation \ref{eq:arm-pull-opt}, we can bound the probability of its complementary event by,

\begin{align*}
\sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\sum_{n_{i*}=1}^{\ell_{m_{}}}\Pb\lbrace s_i < s_{i*}\rbrace \leq \sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\sum_{n_{i*}=1}^{\ell_{m_{}}}\Pb\lbrace n_i > n_{i*}\rbrace \leq \sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\sum_{n_{i*}=1}^{\ell_{m_{}}}\Pb\lbrace \hat{r}_{i,c_j} + s_i > \hat{r}_{i*,c_j} + s_{i*} \rbrace.
\end{align*}

But the event $\hat{r}_{i,c_j} + s_i > \hat{r}_{i*,c_j} + s_i$ is possible only when the following three events occur, $\hat{r}_{i*,c_j} \leq r_{i*,c_j} - s_{i*} , \hat{r}_{i,c_j} \geq r_{i,c_j} + s_i$ and $r_{i*}-r_{i} < 2(1+\gamma)^2 s_i $. But the third event will not happen for $n_i\geq \ell_{m_{i,c_j}}$. Proceeding as before, we can show that the probability of the remaining two events is bounded by,

\begin{align*}
&\sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\sum_{n_{i*}=1}^{\ell_{m_{}}}\Pb\lbrace s_i < s_{i*}\rbrace \leq \sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\sum_{n_{i*}=1}^{\ell_{m_{}}}\Pb\lbrace n_i > n_{i*}\rbrace \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
& \leq \sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\sum_{n_{i*}=1}^{\ell_{m_{}}}\Pb\lbrace \hat{r}_{i,c_j} + s_i > \hat{r}_{i*,c_j} + s_{i*} \rbrace \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\leq \sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\sum_{n_{i*}=1}^{\ell_{m_{}}}\left( \Pb\lbrace \hat{r}_{i,c_j} \geq r_{i,c_j} + s_i \rbrace \bigcup \Pb\lbrace \hat{r}_{i*,c_j} \leq r_{i*,c_j} - s_{i*} \rbrace \right)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\leq \sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\left( \Pb\lbrace \hat{r}_{i,c_j} \geq r_{i,c_j} + s_i \rbrace \right) +  \sum_{m=0}^{m_{i,c_j}}\sum_{n_{i*}=1}^{\ell_{m_{}}}\left( \Pb\lbrace \hat{r}_{i*,c_j} \leq r_{i*,c_j} - s_{i*} \rbrace \right) \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\leq \sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\dfrac{1}{\psi T\epsilon_{m_{}}^2} +  \sum_{m=0}^{m_{i,c_j}}\sum_{n_{i*}=1}^{\ell_{m_{}}}\dfrac{1}{\psi T\epsilon_{m_{}}^2} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\leq 2\left(\dfrac{\log(\psi T \epsilon_{m_{i,c_j}}^2)}{2(\psi T)^{\alpha}}\right)\sum_{m=0}^{m_{i,c_j}}\dfrac{1}{\epsilon_{m_{}}^{2\alpha + 1}}.
\end{align*}

%\sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{i,c_j}}}
Finally for the fourth event in equation \ref{eq:arm-pull-opt}, we can bound the probability of its complementary event by following the same steps as above,

\begin{align*}
\sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\sum_{n_{i*}=1}^{\ell_{m_{}}}\Pb\lbrace n_i > n_{i*}\rbrace &\leq \sum_{m=0}^{m_{i,c_j}}\sum_{n_i=1}^{\ell_{m_{}}}\sum_{n_{i*}=1}^{\ell_{m_{}}}\Pb\lbrace r_{i,c_j} + s_i > r_{i*,c_j} + s_{i*} \rbrace\\
%%%%%%%%%%%%%%%%%%%%%%%%%%
&\leq \dfrac{\log(\psi T \epsilon_{m_{i,c_j}}^2)}{(\psi T)^{\alpha}}\sum_{m=0}^{m_{i,c_j}}\dfrac{1}{\epsilon_{m}^{2\alpha +1}}.
\end{align*}


Combining the above four cases we can bound the probability that a sub-optimal arm $i$ will no longer be pulled on or after the $m_{i,c_j}$-th phase by,

\begin{align*}
\dfrac{4\log(\psi T \epsilon_{m_{i,c_j}}^2)}{(\psi T)^{\alpha}}\sum_{m=0}^{m_{i,c_j}}\dfrac{1}{\epsilon_{m_{i,c_j}}^{2\alpha +1}} &\leq \dfrac{4\log(\psi T \epsilon_{m_{i,c_j}}^2)}{(\psi T)^{\alpha}}\sum_{m=0}^{M}\left(\dfrac{1}{\epsilon_{m}}\right)^{2\alpha +1}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%
& \overset{(a)}{\leq} \dfrac{4\log(\psi T \epsilon_{m_{i,c_j}}^2)}{(\psi T)^{\alpha}}\left(\dfrac{(1+\gamma)((1+\gamma)^M - 1)}{(1+\gamma) - 1}\right)^{2\alpha +1} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\overset{(b)}{\leq} \dfrac{4\log(\psi T \epsilon_{m_{i,c_j}}^2)}{(\psi T)^{\alpha}}\left( \left( \dfrac{1+\gamma}{\gamma}\right) \sqrt{T}\right)^{2\alpha +1} \overset{(c)}{=} \dfrac{4\sqrt{T}C\left(\gamma, \alpha \right)\log(\psi T \epsilon_{m_{i,c_j}}^2)}{(\psi)^{\alpha}}.
\end{align*}

Here, in $(a)$ we use the standard geometric progression formula, in $(b)$ we substitute the value of $M=\dfrac{1}{2}\log_{1+\gamma}\dfrac{T}{e}$ and in $(c)$ we substitute $C\left(\gamma, \alpha \right)= \left( \dfrac{1+\gamma}{\gamma}\right)^{2\alpha + 1}$ . Bounding this trivially by $T\Delta^{opt}_{i,c_j}$ for each arm $i\in\A'$ we get the regret suffered for all arm $i\in\A'$ after the $m_{i,c_j}$-th phase  as,

\begin{align*}
\sum_{i\in\A'}\left( \dfrac{4T\Delta^{opt}_{i,c_j}\sqrt{T}C_{\gamma}\log(\psi T \epsilon_{m_{i,c_j}}^2)}{(\psi)^{\alpha}} \right) \leq \sum_{i\in\A'}\left( \dfrac{4T^{\frac{3}{2}}C\left(\gamma, \alpha \right)\Delta^{opt}_{i,c_j}\log(\psi T (\Delta^{opt}_{i,c_j})^4)}{(\psi)^{\alpha}} \right).
\end{align*}


%\begin{align*}
%\sum_{i\in\A}\left(\dfrac{4T\Delta^{opt}_{i,c_j}\log(\psi T)}{(\psi T)^{\alpha}}\sum_{m=0}^{m_{i,c_j}}\dfrac{1}{\epsilon_{m_{i,c_j}}^{2\alpha +1}}\right) \leq \sum_{i\in\A}\left(\dfrac{4T\Delta^{opt}_{i,c_j}\log(\psi T)}{(\psi T)^{\alpha}}\dfrac{M 2^{2\alpha +1}}{(\Delta^{opt}_{i,c_j})^{4\alpha +2}}\right).
%\end{align*}

\textbf{Step 5.(Regret for pulling the sub-optimal arm $i$ on or before $m_{i,c_j}$-th phase):} Either a sub-optimal arm gets pulled $\ell_{m_{i,c_j}}$ number of times till the $m_{i,c_j}$-th phase or after that the probability of it getting pulled is exponentially low (as shown in \textbf{step 4}). Hence, the number of times a sub-optimal arm $i$ is pulled till the $m_{i,c_j}$-th phase is given by,

\begin{align*}
n_i < \ell_{m_{i,c_j}} = \left\lceil \dfrac{\log(\psi T\epsilon_{m_{i,c_j}}^2)}{2\epsilon_{m_{i,c_j}}} \right\rceil
\end{align*}

Hence, considering each arm $i\in\A'$ the total regret is bounded by,

\begin{align*}
\sum_{i\in\A'}\Delta^{opt}_{i,c_j}\left\lceil \dfrac{\log(\psi T\epsilon_{m_{i,c_j}}^2)}{2\epsilon_{m_{i,c_j}}} \right\rceil < \sum_{i\in\A'}\Delta^{opt}_{i,c_j}\left[ 1 + \dfrac{\log(\psi T\epsilon_{m_{i,c_j}}^2)}{2\epsilon_{m_{i,c_j}}} \right] \leq \sum_{i\in\A'}\Delta^{opt}_{i,c_j}\left[ 1 + \dfrac{4\log(\psi T(\Delta^{opt}_{i,c_j})^4)}{(\Delta^{opt}_{i,c_j})^2}\right].
\end{align*} 

\textbf{Step 6.(Regret for not detecting changepoint $c_{j}$ for arm $i$ after the $p_{i,c_j}$-th phase):} First we define a few additional notations, starting with $\hat{r}_{i,N_{p_{i,c_{j-1}}}:N_{m'}}$ denoting the sample mean of the $i$-th arm from $N_{p_{i,c_{j-1}}}$ to $N_{m'}$ timestep while $\hat{r}_{i,N_{m'}+1:N_{p_{i,c_j}}}$ denotes the sample mean of the $i$-th arm from $N_{m'}+1$ to $N_{p_{i,c_j}}$ timesteps where $m'=1,\ldots,p_{i,c_j}$. Proceeding similarly as in \textbf{step 4} we can show that in the $p_{i,c_j}$-th phase for an arm $i\in\A'$ if $n_{i}\geq\ell_{p_{i,c_j}}$ then,

\begin{align*}
s_i = \sqrt{\dfrac{\alpha\log(\psi T\epsilon_{p_{i,c_j}}^2)}{2n_{i}}} \leq \sqrt{\dfrac{\alpha\log(\psi T\epsilon_{p_{i,c_j}}^2)}{2\ell_{p_{i,c_j}}}} \leq \sqrt{\alpha\epsilon_{p_{i,c_j}}\dfrac{\log(\psi T\epsilon_{p_{i,c_j}}^2)}{\log(\psi T\epsilon_{p_{i,c_j}}^2)}} \leq \dfrac{\Delta^{chg}_{i,c_j}}{2(1+\gamma)^2}.
\end{align*}

Furthermore, we can show that for a phase $m\in[1,p_{i,c_j}]$ if the following three conditions hold for an arm $i\in\A'$ then the changepoint will definitely get detected, that is,

\begin{eqnarray}
&\hat{r}_{i,N_{p_{i,c_{j-1}}}:N_{m}} + s_{i,N_{p_{i,c_{j-1}}}:N_{m}} < \hat{r}_{i,N_{m}+1:N_{p_{i,c_j}}} - s_{i,N_{m}+1:N_{p_{i,c_j}}},\hspace*{4mm}
\nonumber\\
&\hat{r}_{i,N_{p_{i,c_{j-1}}}:N_{m}} - s_{i,N_{p_{i,c_{j-1}}}:N_{m}} > \hat{r}_{i,N_{m}+1:N_{p_{i,c_j}}} + s_{i,N_{m}+1:N_{p_{i,c_j}}},\hspace*{4mm} 
\nonumber\\
& s_{i,N_{p_{i,c_{j-1}}}:N_{m}} < s_{i,N_{m}+1:N_{p_{i,c_j}}} \label{eq:arm-pull-chg}.\\\nonumber
\end{eqnarray}

Indeed, we can show that if there is a changepoint at $c_j$ such that $r_{i,c_{j-1}} < r_{i,c_j}$ and if the first and third  conditions in equation \ref{eq:arm-pull-chg} hold  in the $p_{i,c_j}$-th phase then,

\begin{align*}
\hat{r}_{i,N_{p_{i,c_{j-1}}}:N_{m}} + s_{i,N_{p_{i,c_{j-1}}}:N_{m}} &\leq {r}_{i,c_{j-1}} + 2(1+\gamma)^2 s_{i,N_{p_{i,c_{j-1}}}:N_{m}} - (1+\gamma)^2s_{i,N_{p_{i,c_{j-1}}}:N_{m}}\\
%%%%%%%%%%%%%%%%%%%
& \leq {r}_{i,c_{j-1}} + \Delta^{chg}_{i,c_j} - (1+\gamma)^2s_{i,N_{p_{i,c_{j-1}}}:N_{m}}\\
%%%%%%%%%%%%%%%%%%%
 &\leq {r}_{i,c_{j}} - (1+\gamma)^2s_{i,N_{m}+1:N_{p_{i,c_j}}} \leq \hat{r}_{i,N_{m}+1:N_{p_{i,c_j}}} - s_{i,N_{m}+1:N_{p_{i,c_j}}}.
\end{align*}

Conversely, for the case $r_{i,c_{j-1}} > r_{i,c_j}$ the second and third conditions will hold for the $p_{i,c_j}$-th phase. Now, to bound the regret we need to bound the probability of the complementary of these three events. For the complementary of the first event in equation \ref{eq:arm-pull-chg} by using Chernoff-Hoeffding bound we can show that for all $m'\in[1,p_{i,c_j}]$,

\begin{align*}
&\sum_{m=0}^{m'}\sum_{n_i=1}^{\ell_{m'}}\Pb\lbrace \hat{r}_{i,N_{p_{i,c_{j-1}}}:N_{m'}} \geq  r_{i,c_{j-1}} + s_{i,N_{p_{i,c_{j-1}}}:N_{m'}} \rbrace \leq \sum_{m=0}^{p_{i,c_j}}\sum_{n_i=1}^{\ell_{p_{i,c_j}}}\exp\left(-2s_{i}^2n_{i} \right)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\leq \sum_{m=0}^{p_{i,c_j}}\sum_{n_i=1}^{\ell_{m}}\exp\left(-2\dfrac{\alpha\log(\psi T\epsilon_{m}^2)}{2n_{i}}n_{i} \right)\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
&\leq \sum_{m=0}^{p_{i,c_j}}\sum_{n_i=1}^{\ell_{m}}\dfrac{1}{\psi T\epsilon_{m}^2} \leq \sum_{m=0}^{p_{i,c_j}}\dfrac{\log(\psi T\epsilon_{m}^2)}{2\epsilon_{m}}\dfrac{1}{(\psi T\epsilon_{m}^2 )^{\alpha}} \leq  \dfrac{\log(\psi T\epsilon_{p_{i,c_j}}^2)}{2(\psi T)^{\alpha}}\sum_{m=0}^{p_{i,c_j}}\dfrac{1}{\epsilon_{m}^{2\alpha + 1}}.
\end{align*}

Also, again by using Chernoff-Hoeffding bound we can show that for all $m'\in[1,p_{i,c_j}]$,

\begin{align*}
\sum_{m=m'}^{p_{i,c_j}}\sum_{n_i=1}^{\ell_{p_{i,c_j}}}\Pb\lbrace \hat{r}_{i,N_{m'}+1:N_{p_{i,c_j}}} \leq  r_{i,c_j} - s_{i,N_{m'}+1:N_{p_{i,c_j}}} \rbrace &\leq \sum_{m=0}^{p_{i,c_j}}\sum_{n_i=1}^{\ell_{m}}\exp\left(-2s_{i}^2n_{i} \right) \leq \dfrac{\log(\psi T\epsilon_{p_{i,c_j}}^2)}{2(\psi T)^{\alpha}}\sum_{m=0}^{p_{i,c_j}}\dfrac{1}{\epsilon_{m}^{2\alpha + 1}}.
\end{align*}

%\ell_{p_{i-1, c_j}}
Hence, the probability that the changepoint is not detected by the first event in equation \ref{eq:arm-pull-chg} is bounded by,
\begin{align*}
\dfrac{\log(\psi T \epsilon_{p_{i,c_j}}^2)}{(\psi T )^{\alpha}}\sum_{m=0}^{p_{i,c_j}}\dfrac{1}{\epsilon_{m}^{2\alpha + 1}}.
\end{align*}

Similarly, we can bound the probability of the complementary of the second event in equation \ref{eq:arm-pull-chg} for a $m'\in[1,p_{i,c_j}]$ as,

\begin{align*}
&\sum_{m=0}^{m'}\sum_{n_i=1}^{\ell_{m'}}\Pb\lbrace \hat{r}_{i,t_0:N_{m'}} \leq  r_{i,c_{j-1}} - s_{i,t_0:N_{m'}} \rbrace\leq \dfrac{\log(\psi T\epsilon_{p_{i,c_j}}^2)}{2(\psi T)^{\alpha}}\sum_{m=0}^{p_{i,c_j}}\dfrac{1}{\epsilon_{m}^{2\alpha + 1}} \textbf{,  and  }\\
%%%%%%%%%%%%%%%%%%%%%%%%%
&\sum_{m=m'}^{p_{i,c_j}}\sum_{n_i=1}^{\ell_{m'}}\Pb\lbrace \hat{r}_{i,c_j} \geq  r_{i,c_j} + s_i \rbrace\leq \dfrac{\log(\psi T\epsilon_{p_{i,c_j}}^2)}{(\psi T)^{\alpha}}\sum_{m=0}^{p_{i,c_j}}\dfrac{1}{\epsilon_{m}^{2\alpha + 1}}.
\end{align*}

%\ell_{p_{i-1,c_j}}

Combining the contribution from these two events, we can show that the probability of not detecting the changepoint $c_j$ for the $i$-th arm after the $p_{i,c_j}$-th phase is upper bounded by,

\begin{align*}
\dfrac{2\log(\psi T)}{(\psi T\epsilon_{p_{i,c_j}}^2)^{\alpha}}\sum_{m=0}^{p_{i,c_j}}\dfrac{1}{\epsilon_{p_{i,c_j}}^{2\alpha + 1}} \overset{(a)}{\leq} \dfrac{2C\left(\gamma,\alpha\right)\sqrt{T}\log(\psi T \epsilon_{p_{i,c_j}}^2)}{(\psi)^{\alpha}} .
\end{align*}

Here, in $(a)$ we substitute $C\left(\gamma,\alpha\right)=\left( \dfrac{1+\gamma}{\gamma}\right)^{2\alpha + 1}$ and we follow the same steps as in \textbf{step 4} to reduce the expression to the above form. Furthermore, bounding the regret trivially (after the changepoint $c_j$) by $\Delta^{opt}_{i,c_{j+1}}$ for each arm $i\in\A'$, we get 


\begin{align*}
\sum_{i\in\A'}\left( \dfrac{2T\Delta^{opt}_{i,c_{j+1}}\sqrt{T}C\left(\gamma,\alpha\right)\log(\psi T \epsilon_{p_{i,c_j}}^2)}{(\psi)^{\alpha}} \right) \leq \sum_{i\in\A'}\left( \dfrac{2T^{\frac{3}{2}}C\left(\gamma,\alpha\right)\Delta^{opt}_{i,c_{j+1}}\log(\psi T (\Delta^{chg}_{i,c_j})^4)}{(\psi)^{\alpha}} \right).
\end{align*}


%\begin{align*}
%\sum_{i\in\A}\left(\dfrac{2T\Delta^{opt}_{i,c_{j+1}}\log(\psi T)}{(\psi T)^{\alpha}}\sum_{m=0}^{p_{i,c_j}}\dfrac{1}{\epsilon_{p_{i,c_j}}^{2\alpha + 1}}\right) \leq \sum_{i\in\A}\left(\dfrac{2T\Delta^{opt}_{i,c_{j+1}}\log(\psi T)}{(\psi T)^{\alpha}}\dfrac{M 2^{2\alpha + 1}}{(\Delta^{chg}_{i,c_j})^{4\alpha + 2}}\right).
%\end{align*}

\textbf{Step 7.(Regret for not detecting a changepoint $c_{j}$ for arm $i\in\A$ on or before the $p_{i,c_j}$-th phase):} The regret for not detecting the changepoint $c_j$ on or before the $p_{i,c_j}$-th phase can be broken into two parts, \textbf{(a)} the worst case events from $t_{c_j}$ to $p_{i}$ and \textbf{(b)} the minimum number of pulls $\ell_{p_{i,c_j}}$ required to detect the changepoint. For the first part (a) we can use Assumption \ref{assm:space-gap}, Assumption ref{assm:chg-gap}, Discussion \ref{dis:gap-delay} and Definition \ref{Def:e-chg-gap} to upper bound the regret as,

\begin{align*}
\sum_{i\in\A}\Delta^{opt}_{\max,c_{j+1}}\left\lceil \dfrac{\log(\psi T\epsilon_{p_{i,c_j}}^2)}{2(\Delta^{chg}_{\epsilon_0,c_j})^2} \right\rceil < \sum_{i\in\A}\Delta^{opt}_{\max,c_{j+1}}\left[ 1 + \dfrac{\log(\psi T\epsilon_{p_{i,c_j}}^2)}{2(\Delta^{chg}_{\epsilon_0,c_j})^2} \right].
\end{align*}

Again, for the second part (b) the arm $i\in\A'$ can be pulled no more than $\ell_{p_i}$ number of times. Hence, for each arm $i\in\A$  the regret for this case is bounded by,

\begin{align*}
\sum_{i\in\A'}\Delta^{opt}_{i,c_{j+1}}\left\lceil \dfrac{\log(\psi T\epsilon_{p_{i,c_j}}^2)}{2\epsilon_{p_{i,c_j}}} \right\rceil <  \sum_{i\in\A'}\Delta^{opt}_{i,c_{j+1}}\left[ 1 + \dfrac{\log(\psi T\epsilon_{p_{i,c_j}}^2)}{2\epsilon_{p_i}} \right].
\end{align*}

Therefore, combining these two parts (a) and (b) we can show that the total regret for not detecting the changepoint till the $p_{i,c_j}$-th phase is given by,

\begin{align*}
&\sum_{i\in\A}\left\lbrace\Delta^{opt}_{\max,c_{j+1}} + \dfrac{\Delta^{opt}_{\max,c_{j+1}}\log(\psi T\epsilon_{p_{i,c_j}}^2)}{2(\Delta^{chg}_{\epsilon_0,c_j})^2}\right\rbrace + \sum_{i\in\A'}\left\lbrace\Delta^{opt}_{i,c_{j+1}} + \dfrac{\Delta^{opt}_{i,c_{j+1}}\log(\psi T\epsilon_{p_{i,c_j}}^2)}{2\epsilon_{p_{i,c_j}}}\right\rbrace \\
%%%%%%%%%%%%%%%%%%%%%%%%%
&\leq \sum_{i\in\A}\left\lbrace\Delta^{opt}_{\max,c_{j+1}} + \dfrac{4\Delta^{opt}_{\max,c_{j+1}}\log(\psi T(\Delta^{chg}_{i,c_j})^4)}{(\Delta^{chg}_{\epsilon_0,c_j})^2} \right\rbrace + \sum_{i\in\A'}\left\lbrace \Delta^{opt}_{i,c_{j+1}} + \dfrac{4\Delta^{opt}_{i,c_{j+1}}\log(\psi T(\Delta^{chg}_{i,c_j})^4)}{(\Delta^{chg}_{i,c_j})^2}\right\rbrace
\end{align*}

\textbf{Step 8.(Final Regret bound):} Combining the assumption in \textbf{Step 0} and the problem definition, the expected regret till the $T$-th timestep is bounded by,

\begin{align*}
\E[R_{T}]&= \sum_{i = 1}^K\sum_{j=1}^{G}\Delta^{opt}_{i,c_j}\E[n_{i_j\neq i^*_{j}}] \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%
& \leq \sum_{i\in\A'}\sum_{j=1}^{G}\bigg[ 1 
%%%%%%%%%%
+ \underbrace{ \dfrac{4T^{\frac{3}{2}}C\left( \gamma,\alpha\right)\Delta^{opt}_{i,c_j}\log(\psi T (\Delta^{opt}_{i,c_j})^4)}{(\psi)^{\alpha}} }_{\textbf{from Step 4}}
%%%%%%%%%%
+ \underbrace{\Delta^{opt}_{i,c_j} + \dfrac{4\log(\psi T(\Delta^{opt}_{i,c_j})^4)}{(\Delta^{opt}_{i,c_j})}}_{\textbf{from Step 5}}\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%
& + \underbrace{ \dfrac{2T^{\frac{3}{2}}C\left( \gamma,\alpha\right)\Delta^{opt}_{i,c_{j+1}}\log(\psi T (\Delta^{chg}_{i,c_j})^4)}{(\psi)^{\alpha}} }_{\textbf{from Step 6}}\bigg]\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%
&+ \underbrace{ \sum_{i\in\A}\sum_{j=1}^{G}\bigg[\Delta^{opt}_{\max,c_{j+1}} + \dfrac{4\Delta^{opt}_{\max,c_{j+1}}\log(\psi T(\Delta^{chg}_{i,c_j})^4)}{(\Delta^{chg}_{\epsilon_0,c_j})^2}\bigg] + \sum_{i\in\A'}\sum_{j=1}^{G}\bigg[\Delta^{opt}_{i,c_{j+1}} + \dfrac{4\Delta^{opt}_{i,c_{j+1}}\log(\psi T(\Delta^{chg}_{i,c_j})^4)}{(\Delta^{chg}_{i,c_j})^2}}_{\textbf{from Step 7}}
\bigg]
\end{align*}

Hence, we get the main result of the regret bound.

\end{customproof}



==> related.tex <==
Existing algorithms for the piecewise i.i.d bandit setting can be broadly divided into two categories, passively adaptive and actively adaptive strategies. Passively adaptive strategies like Discounted UCB (DUCB) \citep{kocsis2006discounted}, Sliding Window UCB (SWUCB) \citep{garivier2011upper} and Discounted Thompson Sampling (DTS) \citep{raj2017taming} do not actively try to locate the changepoints but rather try to minimize their losses by focusing on past few observations. In \citet{garivier2011upper} the authors showed that the regret upper bound of DUCB and SWUCB are respectively $O( \sqrt{GT}\log T)$ and $O(\sqrt{GT\log T} )$, where $G$ is the total number of changepoints and $T$ is the time horizon which are known apriori. Furthermore, \citet{garivier2011upper} proved that the cumulative regret in this setting for a policy $\pi$ for two changepoints   is lower bounded in the order of $\Omega( \sqrt{T})$. The actively adaptive strategies like Adapt-EVE \citep{hartland2007change}, Windowed-Mean Shift \citep{yu2009piecewise}, EXP3.R  \citep{allesiardo2017non}, CUSUM \citep{liu2017change} try to locate the changepoints and restart the chosen bandit algorithms. The regret bound of Adapt-EVE and DTS is still an open problem, whereas the regret upper bound of EXP3.R is $O(G\sqrt{T\log T})$ and that of CUSUM is $O( \sqrt{GT\log({T}/{G})})$. The regret bound of CUSUM is restricted to only Bernoulli distributions. We also implement two oracle algorithms, Oracle UCB1 (OUCB1) and Oracle Thompson Sampling (OTS) which are actively adaptive algorithms with the knowledge of the changepoints. They are restarted at the changepoints without any delay with all their past history of actions and rewards erased. OUCB1  has a regret upper bound of $O(\sqrt{GT\log({T}/{G})})$ (see Proposition \ref{psbandit:Prop:1}, Appendix \ref{proof:Proposition:1}). An extended discussion on related work can be found in Appendix \ref{sec:appendix:related}.

%We further provide a refined lower bound for an optimal oracle policy $\pi^*$ that scales as $\Omega(\sqrt{GT})$ which none of the current algorithms are able to reach.
%Hence, none of the algorithms reaches the lower bound as proved by \citet{garivier2011upper}.
%and OTS have the same regret upper bound of $O(\sqrt{GT\log \frac{T}{G}})$ but empirically outperforms OUCB1
%So both of these oracle algorithms have the worst case regret upper bound larger than the lower bound $\Omega( \sqrt{T})$ proven by  \citet{garivier2011upper}.
%Furthermore, there are the oracle algorithms which are adaptive algorithms having access to the changepoints and can be treated as baseline algorithms. Hence, they are restarted at the changepoints without any delay with all their past history of actions and rewards erased. We implement two Oracle algorithms, Oracle UCB1 (OUCB1) and Oracle Thompson Sampling (OTS). OUCB1  has a regret upper bound of $(\sqrt{GT\log \frac{T}{G}})$ and OTS have the same regret upper bound of $(\sqrt{GT\log \frac{T}{G}})$ but empirically outperforms OUCB1. Note, that both of these Oracle algorithms have the worst case regret upper bound larger than the lower bound $\Omega( \sqrt{T})$ proven by  \citet{garivier2011upper}. Hence, none of the algorithms reaches the lower bound as proved by \citet{garivier2011upper}. An extended discussion on related work can be found in \ref{sec:appendix:related}.

